Lipschitz-Margin Training: Scalable Certification of Perturbation Invariance for Deep Neural Networks

High sensitivity of neural networks against malicious perturbations on inputs causes security concerns. To take a steady step towards robust classifiers, we aim to create neural network models provably defended from perturbations. Prior certification work requires strong assumptions on network structures and massive computational costs, and thus the range of their applications was limited. From the relationship between the Lipschitz constants and prediction margins, we present a computationally efficient calculation technique to lower-bound the size of adversarial perturbations that can deceive networks, and that is widely applicable to various complicated networks. Moreover, we propose an efficient training procedure that robustifies networks and significantly improves the provably guarded areas around data points. In experimental evaluations, our method showed its ability to provide a non-trivial guarantee and enhance robustness for even large networks.

==> related_work.tex <==

    \section{Related work}
    One approach to defend from adversarial perturbations is to regularize or mask gradients.
    Defensive distillation \citep{DefensiveDistillation}, which distills networks into themselves, is one of the most prominent methods.
    However, \citet{CW} showed that we can create adversarial perturbations that deceive networks trained with defensive distillation.
    Input transformations and detections \citep{FeatureSqueezing, InputTransform} are some other defense strategies, although we can bypass them \citep{Bypassed}.
    Adversarial training \citep{FGSM, AtScale, Madry}, which injects adversarially perturbed data into training data, is a promising approach.
    However, there is a risk of overfitting to attacks \citep{AtScale, Ensemble}.
    Note that these kinds of techniques are orthogonal to the algorithms proposed in this paper.

    The existing literature indicates the difficulty in evaluation of the robustness.
    Several studies addresses this difficulty.
    One of the popular approaches is restricting discussion to networks using ReLU \citep{ReLU} exclusively as their activation functions and reducing the verification problem to some other well-studied problems.
    \citet{LP} encoded networks to linear programs, \citet{ReluPlex, TowardsProving} reduced the problem to Satisfiability Modulo Theory, and \citet{SDP} encoded networks to semidefinite programs.
    However, these formulations demand prohibitive computational costs and their applications are limited to only small networks.
    As a relatively tractable method, \citet{OuterPolytope} have bounded the influence of $\ell_\infty$-norm bounded perturbations using convex outer-polytopes.
    However, it is still hard to scale this method to deep or wide networks.
    Another approach is assuming smoothness of networks and losses.
    \citet{FormalGuarantee} focused on local Lipschitz constants of neural networks around each input.
    However, the guarantee is provided only for networks with one hidden layer.
    \citet{LowerBounds} lower-bounded the size of adversarial perturbations that can never deceive networks in a layer-wise manner.
    \citet{DistributionalRobustness} proposed a certifiable procedure of adversarial training.
    However, smoothness constants, which their certification requires, are usually unavailable or infinite.
    \citet{Extreme} proposed to estimate a Lipschitz constant of networks, while it fails to provide certification \citep{ExtremeRebuttal}.
    As a concurrent work, \citet{Reachability} proposed another algorithm to certify robustness with more scalable manner than previous approaches.
    However, it requires that the Lipschitz constant is given, and this work complements it.
    We also note that our algorithm is still significantly faster and more widely applicable.

    Our work is an extension of \citet{Intriguing} and its subsequent work: Parseval networks \citep{Parseval}.


